Facing Device Attribution Problem for Stabilized Video Sequences

A problem deeply investigated by multimedia forensics researchers is the one of detecting which device has been used to capture a video. This enables to trace down the owner of a video sequence, which proves extremely helpful to solve copyright infringement cases as well as to fight distribution of illicit material (e.g., underage clips, terroristic threats, etc.). Currently, the most promising methods to tackle this task exploit unique noise traces left by camera sensors on acquired images. However, given the recent advancements in motion stabilization of video content, robustness of sensor pattern noise-based techniques are strongly hindered. Indeed, video stabilization introduces geometric transformations between video frames, thus making camera fingerprint estimation problematic with classical approaches. In this paper, we deal with the challenging problem of attributing stabilized videos to their recording device. Specifically, we propose: (i) a strategy to extract the characteristic fingerprint of a device, starting from either a set of images or stabilized video sequences; (ii) a strategy to match a stabilized video sequence with a given fingerprint in order to solve the device attribution problem. The proposed methodology is tested on videos coming from a set of different smartphones, taken from the modern publicly available Vision Dataset. The conducted experiments also provide an interesting insight on the effect of modern smartphones video stabilization algorithms on specific video frames.

==> alg_Ki.tex <==
\subsection{Reference PRNU from flat-field images}
\label{subsec:alg_Ki}

This Section is inspired to some related work presented in \cite{iuliani2017}. 
In their paper, authors compute the reference PRNU for each source exploiting flat-field images shot by the corresponding camera. 
In this case, the PRNU, defined as $ \hKi $, is estimated following the pipeline proposed by \cite{Chen2008} and reported in eq. \eqref{eq:prnu_def}.

%%% dal dominio dell'img a quello del video 
Actually, $ \hKi $ cannot be directly exploited for solving the source attribution problem on video sequences. 
As a matter of fact, during video recording, some scaling and cropping operations are performed, in order to reduce the recording area and to adapt the sensor size to the desired aspect ratio, which is typically 16:9 for videos. 
Formally, the image-to-video conversion can be modeled with the series of two steps, which are:
\begin{enumerate}
	\item a scaling operation, in order to shrink the image content over a reduced pixel area;
	\item a cropping operation, in order to match the desired dimensions of the video sequence.
\end{enumerate}

For the sake of clarity, Fig.~\ref{fig:I_to_V_conv} depicts the relationship between image resolution ($ X_{\mathrm{I}} \times Y_{\mathrm{I}} $) and video resolution ($ X_{\mathrm{V}} \times Y_{\mathrm{V}} $). $\Si$ represents the scaling factor applied in image domain, while $ \Cix$ and $ \Ciy $ are the parameters related to the cropping operation, namely the horizontal and vertical coordinates of the upper-left corner pixel of the video area. 

\begin{figure}[t]
	\centering
	\includegraphics[width=.6\columnwidth]{figures/I_to_V_conv.pdf}
	\caption{Example of sensor area reduction in video acquisition. Blue area represents the whole sensor size, used for images, while gray area is the final area for video acquisition. }
	\label{fig:I_to_V_conv}
\end{figure}

As a consequence, it is not possible to directly compare the fingerprint $ \hKi $ with the video sequences. 
In order to perform the comparison, we need to register the estimated PRNU into the video domain.
Since every device is characterized by its own scaling and cropping parameters, these can be actually estimated exploiting both captured images and videos. 

%%% spiegazione del passaggio img-video, con la stima dei parametri con PSO
To be more precise, let us describe the process for a single camera, being the very same for all devices.  
In case of in-camera DVS, we acquire stabilized sequences only, as DVS usually cannot be switched off in an easy way. Hence, the scaling and cropping factors to be applied to $ \hKi $ can be estimated exploiting only stabilized frames. In particular, it can be a proper choice to select an easily manageable sequence, e.g., an almost flat and static video recorded by the camera. 

For each device, we search the factors $ \Si,  \Ci = \{ \Cix, \Ciy \} $ such that the warped version by similarity transformation of $ \hKi $ better correlates on average with the video frames.
To be precise, after selecting a reasonable research-range $ \mathcal{S} $ and $ \mathcal{C} $, we estimate $ \Si_f, \Cix_f$ and $ \Ciy_f $ per each I-frame $ \I_f, \, f \in [1, F]$, solving a maximization problem:
\begin{equation}
\Si_f, \Ci_f= \underset{\S \in \mathcal{S}, \C \in \mathcal{C}}{\arg \max} \,  \mathrm{PCE}(\W_f, \I_f \cdot \mathscr{T}_{\S \C}(\hKi)), 
\label{eq: max_pce}
\end{equation}
where $ \W_f$ is the noise residual extracted from the I-frame $\I_f$, $ \mathscr{T}_{\S \C}(\cdot) $ is the similarity transformation applied to $ \hKi $, and the product $  \I_f \cdot \mathscr{T}_{\S \C}(\hKi) $ is performed pixel-wise. In particular, $ \mathscr{T}_{\S \C}(\cdot) $ is the geometric transformation which applies isotropic scaling and translation, represented by the matrix
\begin{equation}
\mathbf{T}_{\S \C} = \begin{pmatrix}
\S &0  &\Cx\\ 
0 &\S  &\Cy 
\end{pmatrix}.
\end{equation}

In other words, we are searching the geometric transformation $ \mathscr{T}_{\S \C}(\cdot) $ which registers at best $ \hKi $ on the video I-frames, maximizing their correlation in terms of relative PCE. 
%Computing PCE is like solving the source attribution problem for I-frames with respect to the transformed fingerprint $ \mathscr{T}_{s}(\Ki) $. 
%The peak of correlation is searched over all the pixel positions inside the video area $ X_{\mathrm{V}} \times Y_{\mathrm{V}} $.

Due to in-camera DVS, these parameters can vary in time, hence we determine the average parameters over the I-frames of the selected video.
In particular, we average the estimated parameters only for those I-frames who would be attributed to the camera with fingerprint $ \K = \mathscr{T}_{\Si_f \Ci_f}(\hKi) $ in a common attribution problem. Hence, we select only I-frames whose related maximum PCE overcomes a reasonable threshold, i.e., 60 as suggested in \cite{entrieri2016,taspinar2016}:
\begin{equation}
{\Si} =  \sum_{f \in \mathcal{F}_\mathrm{I}} \Si_f \Big / |\mathcal{F}_\mathrm{I}|, 
\end{equation}
and 
\begin{equation}
\Cix =  \sum_{f \in \mathcal{F}_\mathrm{I}} \Cix_f \Big / |\mathcal{F}_\mathrm{I}| \quad \mathrm{and} \quad \Ciy =  \sum_{f \in \mathcal{F}_\mathrm{I}} \Ciy_f \Big / |\mathcal{F}_\mathrm{I}| ,
\end{equation}
being $\mathcal{F}_\mathrm{I}$ the set of selected frames and  $ |\mathcal{F}_\mathrm{I}|$ its cardinality. 

%%% motivare meglio l'utilizzo del PSO
In particular, we use Particle Swarm Optimization (PSO) to perform a global search of the best registration parameters. 
To be precise, we exploit PSO for selecting the best scale parameter, whereas the peak of correlation (related to the cropping factor) is searched over all the pixel positions inside the video area $ X_{\mathrm{V}} \times Y_{\mathrm{V}} $.
As a matter of fact, we noticed that a standard grid search algorithm would be very inefficient for solving the maximization problem, because of the difficulty in setting the grid step for the scale.
Being PSO a global optimization method, we can perform an exhaustive search without sampling the parameter space, just imposing constraints on the research range. 

%%% spiegazione finale del passaggio
In order to pass from image to video domain, we have to apply the similarity transformation $ \mathscr{T}_{\Si \Ci}(\cdot)$ to $\hKi $. We define the obtained PRNU as $ \hKiv $.
Being computed from manifold flat-field images shot by the camera, $ \hKiv $ is reasonably the best PRNU estimation we can achieve. 

%For each device, we search the factors $ \bar{S} $ such that the scaled and translated version by similarity transformation of $ \hKi $ better correlates on average with the video frames.
%To be precise, after selecting a reasonable research-range $ \mathcal{S} $ for the scale, we estimate the scaling factor $ s_f $ per each I-frame $ \I_f, \, f \in [1, F]$, solving a maximization problem:
%\begin{equation}
%s_f = \arg \underset{s \in \mathcal{S}}{\max} \,  \mathrm{PCE}(\W_f, \I_f \cdot \mathscr{T}_{s}(\Ki)) \, , 
%\label{eq: max_pce}
%\end{equation}
%where $ \W_f$ is the noise residual extracted from the I-frame $\I_f$, $ \mathscr{T}_{s}(\cdot) $ is the similarity transformation applied to $ \Ki $, and the product $  \I_f \cdot \mathscr{T}_{s}(\Ki) $ is performed pixel-wise. In particular, $ \mathscr{T}_{s}(\cdot) $ is the geometric transformation which applies isotropic scaling, represented by the matrix
%\begin{equation}
%\mathbf{T}_s = \begin{pmatrix}
%s &0  &0 \\ 
%0 &s  &0 
%\end{pmatrix} \, .
%\end{equation}
%
%In other words, we are searching the geometric transformation $ \mathscr{T}_{s}(\cdot) $ which registers at best $ \Ki $ on the video I-frames, maximizing their correlation in terms of relative PCE. 
%%Computing PCE is like solving the source attribution problem for I-frames with respect to the transformed fingerprint $ \mathscr{T}_{s}(\Ki) $. 
%The peak of correlation is searched over all the pixel positions inside the video area $ X_{\mathrm{V}} \times Y_{\mathrm{V}} $.
%
%Due to in-camera DVS, these parameters can vary in time, hence we determine the average parameters over the I-frames of the selected video.
%In particular, in order to estimate the average scaling $ \bar{s} $, we average the estimated parameters $ s_f $ only for those I-frames who would be attributed to the camera with fingerprint $ \mathscr{T}_{s}(\Ki) $ in a common attribution problem. Hence, we select only I-frames whose related maximum PCE overcomes a reasonable threshold, i.e., 60 as suggested in \cite{entrieri2016,taspinar2016}, and
%\begin{equation}
%\bar{s} =  \sum_{f \in \mathcal{F}_\mathrm{I}} s_f \Big / |\mathcal{F}_\mathrm{I}| \, , 
%\end{equation}
%being $\mathcal{F}_\mathrm{I}$ the set of selected frames and  $ |\mathcal{F}_\mathrm{I}|$ its cardinality. 
%
%For what concerns the average cropping parameters in horizontal and vertical directions, these can be estimated directly from information contained in PCE. 
%Indeed, selecting only I-frames $ f \in \mathcal{F}_\mathrm{I}$, we just need to extract the position of the peak of $ \mathrm{PCE}(\W_f, \I_f \cdot \mathscr{T}_{s_f}(\Ki)) $, obtaining $ c_{f_x} $ and $ c_{f_y} $, the cropping factors on horizontal and vertical directions, respectively. Hence, we average over $\mathcal{F}_\mathrm{I}$:
%\begin{equation}
%\bar{c}_x =  \sum_{f \in \mathcal{F}_\mathrm{I}} c_{f_x} \Big / |\mathcal{F}_\mathrm{I}| \quad \mathrm{and} \quad \bar{c}_y =  \sum_{f \in \mathcal{F}_\mathrm{I}} c_{f_y} \Big / |\mathcal{F}_\mathrm{I}| \, .
%\end{equation}

==> alg_Kv.tex <==
\subsection{Reference PRNU from stabilized video}
\label{subsec:alg_Kv}

Having available information about $ \hKiv  $ is not always straightforward. 
Indeed, you need to have access to images captured by the same device under analysis. 
For this reason, we decided to move away from the solution proposed by \cite{iuliani2017}, trying to estimate the device fingerprint directly from video content. 
%Instead of flat images, for each device, we select a flat and static video for building the reference fingerprint. 
Instead of flat images, we select an easily manageable and almost flat video for building the reference PRNU of each camera.

%%% intro alle 2 sottosezioni
For the sake of clarity, we propose two different computations of the camera PRNU:
\begin{enumerate}[label=\textit{\theenumi)}]
	\item A computation based on an unrealistic situation, albeit very useful for experimental evaluation.
	\item A computation based on a realistic situation, more challenging and complex. 	
\end{enumerate}
We report in the following all the details of the proposed strategies.

\subsubsection{PRNU in presence of oracle}
\label{subsubsec:alg_Kv_o}


In order to proceed step by step, we start building the PRNU in a controlled situation, which is very helpful also to present important considerations regarding DVS. 
Specifically, suppose an oracle gives us information about $ \hKiv  $ for each device, just allowing to exploit it as support for building the fingerprint. 
In order to build the PRNU, we propose to register each of the $ F $ I-frames of the selected video on $ \hKiv $, estimating scale $ S_f $, rotation $ \theta_f $ and translation $ \mathbf{C}_f $ maximizing the relation:
\begin{equation}
S_f, \theta_f, \mathbf{C}_f = \underset{S \in \mathcal{S}, \theta \in \mathcal{T}, \mathbf{C} \in \mathcal{C}}{\arg \max} \,  \mathrm{PCE}(\mathscr{T}_{S \theta \mathbf{C}}(\W_f), \mathscr{T}_{S \theta \mathbf{C}}(\I_f) \cdot  \hKiv ) ,
\label{eq:max_pce_frame}
\end{equation}
$ \forall f \in [1, F] $. 
In particular, we exploit again PSO as global strategy for selecting the best scale and rotation factors, whereas the shift parameter is estimated by searching the highest PCE peak-location.
$ \mathscr{T}_{S \theta \mathbf{C}}(\cdot) $ is the geometric transformation which implements isotropic scaling and rotation, followed by translation, and it is represented by the matrix
\begin{equation}
\mathbf{T}_{S \theta \mathbf{C}} = \begin{pmatrix}
S \, \cos \theta & -S \, \sin \theta &C_x \\ 
S \, \sin \theta & S \, \cos \theta  &C_y
\end{pmatrix} \, .
\end{equation}

%%% perché facciamo questo?
By means of this operation, we are bringing all video frames into alignment exploiting the best reference ever, which is $ \hKiv $. 
As a consequence, we are sufficiently confident that the set of transformations $ \{ \mathscr{T}_{S_f \theta_f \mathbf{C}_f}(\cdot) \} $ provides the best frame configuration for obtaining an estimate of the camera PRNU from a stabilized video. 
Of course, this is clearly an unrealistic situation, but it is a very powerful investigation tool for evaluating the accuracy of our results. In effect, it gives us the best-ever reference to compare our future performances (evaluated on realistic cases) with. 

%%% qui introduciamo la considerazione riguardo il primo frame
Before going on with the computation of PRNU from aligned video frames, some comments should be kept in mind. 
During our experiments, we noticed that the maximum PCE obtained in eq. \eqref{eq:max_pce_frame} presents, on average, higher values on the first video frame $ \I_1 $ than all the others. 
This phenomenon can be explained by the fact that, probably, the effect of DVS in many devices does not immediately start from the first recorded frame, but the stabilizer counteracts the shaking while recording, leaving the first frame almost untouched. 
For this reason, we decided to put apart the first frame from the set of available frames, as it would excessively bias the results (we will eventually prove this in Section \ref{subsubsec:1fr_res}). 
Hence, from now on, the first frame of every sequence is never used, whether for estimating the PRNU or the query fingerprint as well.
%Note that we do not include the first I-frame, since it exhibits a too strong correlation with $ \hKi  $ and would bias the results.
%In order to estimate the cropping factors, $ c_{x_f} $ and $ c_{y_f} $, these can be picked from the relative peak shift of the maximum PCE value obtained from \eqref{eq:max_pce_frame}. 

%%% calcolo del prnu
In order to compute the PRNU from remaining frames, we select only the registered I-frames with maximum $ \mathrm{PCE} \geq 60 $, we average their noise patterns, estimating the device fingerprint $ \hKvi$ as
\begin{equation}
\hKvi= \sum_{f \in \mathcal{F}_\mathrm{V_I}} \mathscr{T}_{S_f \theta_f \mathbf{C}_f}({\W_f}) \Big / |\mathcal{F}_\mathrm{V_I}| \, ,  
\end{equation}
being $ \mathcal{F}_\mathrm{V_I}$ the set of I-frames with acceptable PCE values. 
From now on, the source attribution problem can be solved by means of $ \hKvi$. 

\subsubsection{PRNU from stabilized video}
\label{subsubsec:alg_Kv_no}

In this case, let us suppose we have no access to the images shot by the device, not even to $ \hKiv  $ for building the reference. 
The only information we dispose is the one available from recorded videos. 

In order to build the PRNU, we have to somehow aggregate the noise patterns of the I-frames. 
We need to start from one I-frame, aggregating step by step the noise residuals related to the others. 
However, the procedure of frame aggregation is not straightforward. Indeed, due to in-camera DVS, frames can be shifted, rotated and slightly scaled one another.
Hence, if we just average the noise patterns, the noise traces left by the camera sensor risk to be superimposed in the wrong way, eventually carrying very few content of the device original fingerprint. 

On the other hand, following the previously depicted solutions, one could think it would be a good idea to estimate the warping parameters relating frames one another, eventually averaging the registered noise residuals. However, the estimated geometric transformation risks to be strongly biased by the texture-related content which is naturally contained in each noise residual. 
As a consequence, we will end up registering frames by basically pursuing the depicted scenes and not the PRNU. 
This situation happens for sure if the video sequence has high texture, but also if only a few of this appears in the frames. 

In order to derive a correct PRNU estimation, we propose to start from a properly selected I-frame and aggregate step by step the remaining I-frames following some straight conditions. 
The proposed pipeline is the following:
\begin{enumerate}[label=\textit{\alph*)}]
	\item Loop over all the video I-frames, except the first one (in accordance with previous considerations). For every $ f \in [2, F] $, select as reference the current I-frame $ \I_f $, and solve the standard camera attribution problem for the other I-frames with respect to the reference noise residual $ \W_f $. 
	Specifically, we build the matrix $ \mathbf{P} \in \mathbb{R}^{F-1 \times F-1} $ such that
	\begin{equation}
	\left[\mathbf{P}\right]_{f, l}=  \mathrm{PCE}(\W_l, \I_l \cdot  \W_f) , \quad f, l \in [2, F], \, l \ne f.
	\label{eq:pce_frames_mat}
	\end{equation}
	\item Impose some constraints on the PCE.
	%	\begin{itemize}
	%		\item Consider the only entries of $ \mathbf{P} $ which are in between $ 0 $ and a maximum value, i.e., $ \mathrm{P}_{\mathrm{max}} $. This is done in order to exclude very low correlating frames, but also not to consider strongly correlated frames. As a matter of fact, high values of PCE may be due to scene-content correlation, and can mislead the estimation of the fingerprint. We found out $ \mathrm{P}_{\mathrm{max}} = 2000 $ to be a reasonable maximum value for PCE.
	%		\item 	
	%		We need to make another consideration. 
	
	First, consider only strictly positive PCE values, in order to avoid strongly uncorrelated frames. 
	
	Then, set some conditions on the relative shift between frames.
	As a matter of fact, the effect of in-camera DVS is to rotate, translate and scale the frames one another, but without introducing visible artifacts on the recorded video. 
	For this reason, DVS cannot shift too much one frame with respect to the temporally adjacent ones. 
	
	Formally, if the video was not stabilized, the relative shift $ \mathbf{C}_{fl}$ (estimated from the location of the highest PCE peak) between I-frames $ \I_f $ and $\I_l$ should be of $ \{ 0, 0 \} $ pixels, since both the frames are aligned by their noise residual content.  
	Therefore, in stabilized videos, if the relative alignment $ \mathbf{C}_{fl}$ is too far from $ \{ 0, 0 \} $ position, it means that the PCE peak is mainly due to correlating textured content or additional noise contributions, and not to correlation between the noise patterns related to the original camera fingerprint. 
	Thus, in order to avoid false high correlation results which do not actually correspond to noise residuals'alignment, we limit the research of relative shift between one frame and the others to $ \{ \Delta, \Delta \} $ pixels, e.g., $ \Delta = \{5, 10, 20, 30\}$ in our experiments. 
	%	\end{itemize}
	\item Select as reference frame the I-frame $ \I_f $ with the highest number of correlating frames which follow the reported conditions. 
	The noise pattern $ \W_f $ is the starting reference for building the fingerprint, hence  $ \hK = \W_f$.
	\item Register the frames correlating with $ \hK $, just by translating them of the relative shift estimated by the PCE peak-location. Average their noise patterns in a pixel-wise fashion, building an updated version of the reference $ \hK $,
	\begin{equation}
	\hK = \overline{(\hK, \mathscr{T}_{\mathbf{C}_f} (\W_{f \in \mathcal{F}_\mathrm{V}}) )} \, . 				
	\end{equation}
	$ \mathcal{F}_\mathrm{V}$ is the set of I-frames with acceptable PCE values, while $ \overline{(\cdot)} $ represents the pixel-wise mean. 
	Once included in the computation of $ \hK $, frames are no more used by the algorithm.	
	\item Loop on the remaining I-frames, including them in $  \mathcal{F}_\mathrm{V} $ set if and only if the relative shift with respect to the updated $ \hK $ honors the constraints (i.e., $ C_x \leq \Delta $ and $ C_y \leq \Delta $).
	\item Iterate steps \textit{(d)} and \textit{(e)} until no more frames satisfy the conditions.
	Finally, the estimated device fingerprint is $ \hKv = \hK$. 
\end{enumerate}

%In order to prove our considerations about limiting the relative shift between frames to $ \Delta $ pixels, we investigate in Fig.~\ref{fig:ncc_F_D29_Kv} the behaviour of the cumulative normalized cross-correlation (NCC) between the cumulative estimated $ \hKv $ and the oracle fingerprint $ \hKi $ for one specific camera of the dataset. Fig.~\ref{fig:ncc_F_D29_Kv} depicts cumulative NCC as function of different $ \Delta $ used for the process of frame selection. 
%
%\begin{figure}[b]
%	\centering
%	\includegraphics[width=.8\columnwidth]{figures/ncc_F_D29_Kv}
%	\caption{Normalized cross-correlation NCC between $ \hKv $ and $ \hKi $, vs number of frames used for building the reference.}
%	\label{fig:ncc_F_D29_Kv}
%\end{figure}
%
%We notice that, as $ \Delta $ increases, the cumulative NCC can decrease: this is the sign of the presence of scene correlation between frames, not due to the true PRNU of the camera. 









==> alg_nowarp.tex <==
\subsection{When plenty of frames is available}
\label{subsec:alg_nowarp}

In order to compute the query-video fingerprint when a considerable amount of video frames is available (the accurate meaning of ``considerable'' can be found in Section \ref{subsubsec:alg_nowarp_res}), we propose one possible solution, very efficient and computationally fast. 
Specifically, given a generic PRNU $ \K$, we suggest to solve the standard camera-attribution problem for every frame, without considering any kind of frame registration.
%We compute $\mathrm{PCE}(\W_f, \I_f \cdot \K) $ per each frame of the video. 
In order to attribute or not the video to the camera, we simply select the highest PCE value over the frame-set:
\begin{equation}
P_{test} = \arg \underset{f \in [2, F]}{\max} \, \mathrm{PCE}(\W_f, \I_f \cdot \K).
\label{eq:K_img_nowarp_no1fr}
\end{equation}

We can exploit the variable $P_{test}$ for computing the Receiver Operating Characteristic (ROC) curve of the camera attribution problem as later described in Section \ref{subsubsec:roc}.
By varying the number of frames $ F $, the behaviour of the ROC curve actually changes. Intuitively, the larger the frame-set, the higher the probability to find one correlating frame over the whole video query. 
We will later show how the proposed solution can be very precise, provided some specific requirements. 


%We can exploit the variable $P_{test}$ for computing the Receiver Operating Characteristic (ROC) curve of the camera attribution problem. 
%If we consider an equivalent number of matching and not-matching videos per each source camera, we define as positives the videos where $P_{test} \geq \Gamma$ and negatives the videos with $P_{test}  < \Gamma$. 
%By varying the number of frames, the behaviour of the ROC curve actually changes. Intuitively, the larger the frame-set, the higher the probability to find one correlating frame over the whole video query. We will show in the Result section how the proposed solution can be very precise, provided some specific requirements. 



==> alg_nowarp_res.tex <==
\subsubsection{Query fingerprint from many frames}
\label{subsubsec:alg_nowarp_res}

In this section, we present the ROC curves evaluated on query sequences of $ F $ I-frames, without any geometric transformation applied on them. 
Specifically, we consider videos of different I-frame length, and test this strategy over the estimated camera fingerprints $ \hKiv, \hKvi $ and $ \hKv $.
%In particular, the case $ \hK= \hKvi $ is very useful as upper-bound for the results obtained on $ \hKv $.

Fig.~\ref{fig:ROC_ki_no1fr_nowarp} depicts the results evaluated using $ \hKiv $ as reference. 
We can notice that, for obtaining quite accurate results, sequences of $ 5 $ I-frames are not long enough, while the case $ F = 50 $ achieves very good values. 
In light of this, for testing the reference fingerprints computed from video frames only which are definitely less accurate than $ \hKi $, we opted for investigating the achieved ROC curves using $ 50 $ I-frames, without considering lower values of $ F $. 
%In light of this, regarding the reference fingerprints estimated from video frames only, we tested the sequences using $ 50 $ I-frames, without considering lower values of $ F $. 
Note that some sequences in the dataset do not last until the $ 50 $\textit{-th} I-frame; in these situations we use as many I-frames as available. 

\begin{figure}[t]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/ROC_ki_no1fr_nowarp.pdf}
	\caption{ROC curve exploiting $ \hKi $ as reference fingerprint, testing $ F = \{5, 20, 50\} $ I-frames.}
	\label{fig:ROC_ki_no1fr_nowarp}
\end{figure}

%since the original PRNU content has been already worsened by the fingerprint estimation from the video only.
Fig.~\ref{fig:ROC_kv_kvi_nowarp} depicts the results evaluated on $ \hKvi $ and $ \hKv $. 
%%% considerazioni su Delta. Eliminiamo il caso Delta = 20, e teniamo il 5. ?
In particular, we show the ROC curves corresponding to the different $ \Delta $ exploited for aggregating frames in $ \hKv $ estimation. We can notice that, on average, there is not a noticeable difference between $ \Delta = 5 $ and $ \Delta = 10 $, whereas the case $ \Delta = 20 $ has slightly worse performances.
Anyway, the curves achieved by means of $ \hKv $ can be considered quite accurate if compared with the ROC corresponding to $ \hKvi $. Indeed, the purple line is, at the best of our knowledge, the highest ROC we could compute exploiting video frames for building the reference PRNU. 
Thus, this method has proved to be a valid and efficient strategy for the camera attribution problem, provided the investigated video has a temporal duration of at least $ 30-50 $ seconds. 

\begin{figure}[t]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/ROC_kv_kvi_nowarp.pdf}
	\caption{ROC curve exploiting $ \hKv $ and $ \hKvi $ as reference fingerprint, testing $ F = 50 $ I-frames.}
	\label{fig:ROC_kv_kvi_nowarp}
\end{figure}

To be precise, Table \ref{tab:ki_kv_kvi_nowarp} contains the obtained $ \mathrm{AUC} $ and $ \mathrm{TPR}_{0.01} $ corresponding to all the curves. 
The situation $ \Delta = 20 $ shows lower $ \mathrm{AUC} $ and $ \mathrm{TPR}_{0.01} $, thus we do not consider it in the following investigations. 

%%% dire qualcosa percio sulla lunghezza che deve avere un video? 

\begin{table}[t]
	\caption{$ \mathrm{AUC} $ and $ \mathrm{TPR}_{0.01} $ exploiting $ \hKiv, \hKvi $ and $ \hKv$ as reference fingerprint, testing $ 50 $ I-frames. }
	\label{tab:ki_kv_kvi_nowarp}
	\centering
	\def\arraystretch{1.8}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{c|c|c|c|c|c}
			%			\hline
			$\hK_c$	                        				& $ \hKiv $				& $ \hKvi $   & $ \hKv, \Delta = 5 $     &  $ \hKv, \Delta = 10$      & $ \hKv, \Delta = 20 $  		\\  \Xhline{1.5pt}
			$ \mathrm{AUC} $      				& $ 0.96 $				& $ 0.95 $    & $ 0.88 $                      & $ 0.89 $                     & $ 0.87 $   \\
			 $ \mathrm{TPR}_{0.01} $      & 	$ 0.89 $				& $ 0.83 $    & $ 0.74 $                      & $ 0.75 $                     & $ 0.7 $ \\
			%			\hline
		\end{tabular}}
	\end{table}













==> alg_warp.tex <==
\subsection{If a few video frames is available}
\label{subsec:alg_warp}

When the query video is temporally short, the camera attribution problem cannot be easily solved by the previous methodology, because the few available frames carry little of information about the source PRNU, unless being further processed.
Novel alternative strategies can be proposed. For instance, given a PRNU $ \K$, we propose to solve the camera attribution problem purposely warping the video frames. 
In particular, we aim at estimating the similarity transformation which maximizes the correlation between $ \K$ and the transformed frames. 
Specifically, exploiting PSO, we estimate scale, rotation angle and translation such that:
\begin{equation}
P_f =\underset{S \in \mathcal{S}, \theta \in \mathcal{T}, \mathbf{C} \in \mathcal{C}}{\max} \, \mathrm{PCE}(\mathscr{T}_{S \theta \mathbf{C}}(\W_f), \mathscr{T}_{s \theta \mathbf{C}}(\I_f) \cdot  \K) .
\end{equation}
Then, we select the best $ P_f $ value over all I-frames:
\begin{equation}
P_{test }=\underset{f \in [2, F]}{\max} \, P_f . 
\end{equation}
This approach is actually more accurate than the previously reported, since we are selecting the warping configuration which optimizes at best the correlation with the source camera.
We will later show that a very reduced frame set is necessary for analyzing the query sequence. 
From the other hand, this methodology is slower than the first one, because the estimation of the warping parameters takes some computation time. 



==> alg_warp_res.tex <==
\subsubsection{Query fingerprint from few frames}
\label{subsubsec:alg_warp_res}

%%% alg warp
We report in this section the resulting ROC curves obtained by estimating the geometric transformation which maximizes at best the correlation between $ \hK $ and the video frames. 
To be precise, for each video sequence, we randomly select $ F $ I-frames, testing the method over $ \hKiv, \hKvi $ and $ \hKv $. 

In this case, the parameters estimated by means of PSO has a different research range than in \ref{subsubsec:alg_Ki_res}.
Being all the estimated PRNUs in the same domain of the query, it is not necessary to impose such a wide $ \mathcal{S} $ space. 
As a matter of fact, we aim at \textit{slightly} warping frames, and not at completely disrupting their original content. 
Hence, we select smaller research ranges, i.e., $ \mathcal{S} = [0.99, 1.01] $ and $ \mathcal{T} = [-0.15, 0.15] $ [rad].

Fig.~\ref{fig:ROC_ki_no1fr_warp} depicts the results evaluated using $ \hKiv $ as reference fingerprint. 
We can notice that the method is more accurate than the previous one: as a matter of fact, exploiting just $ 5 $ I-frames (more or less $ 5 $ seconds) returns similar results to the case $ F = 50 $ in absence of warping. 
For this reason, when a few of video frames is available, we suggest to estimate the geometric transformation between the reference fingerprint and the frames, because, at the expense of more computational time, the accuracy can be pretty good. 

\begin{figure}[t]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/ROC_ki_no1fr_warp.pdf}
	\caption{ROC curve exploiting $ \hKiv $ as reference fingerprint, testing $ F = \{1, 5\} $ I-frames.}
	\label{fig:ROC_ki_no1fr_warp}
\end{figure}

When the fingerprint is built directly from the video content, we show results for both $ \hKvi $ and $ \hKv $ in Fig.~\ref{fig:ROC_kv_kvi_warp}. 
Again, there is no evident difference between $ \Delta = 5 $ and $ \Delta = 10 $. Note that, the larger the amount of investigated I-frames, the higher the ROC curve. 
Anyway, even with just $ 5 $ video seconds, we achieve very good accuracies, e.g., $ \mathrm{AUC} \sim 0.90 $.

\begin{figure}[t]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/ROC_kv_kvi_warp.pdf}
	\caption{ROC curve exploiting $ \hKv $ and $ \hKvi $ as reference fingerprint, testing $ F = \{5, 10\} $ I-frames.}
	\label{fig:ROC_kv_kvi_warp}
\end{figure}

More precisely, Table \ref{tab:ki_kv_kvi_warp} contains the obtained $ \mathrm{AUC} $ and $ \mathrm{TPR}_{0.01} $ corresponding to all the curves. 

\begin{table*}[t]
	\caption{$ \mathrm{AUC} $ and $ \mathrm{TPR}_{0.01} $ exploiting $ \hKiv, \hKv $ and $ \hKvi $ as reference fingerprint, testing $ F =\{5, 10\}$ random I-frames. }
	\label{tab:ki_kv_kvi_warp}
	\centering
	\def\arraystretch{1.8}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{c|c|c|c|c|c|c}
			%			\hline
			$\hK_c$	  & $ \hKiv, F = 5 $ & $ \hKvi, F = 5 $   & $ \hKv, \Delta = 5, F = 5 $     &  $ \hKv, \Delta = 5, F = 10$      & $ \hKv, \Delta = 10, F = 5 $  	& $ \hKv, \Delta = 10, F = 10 $ 	\\  \Xhline{1.5pt}
			$ \mathrm{AUC} $      				& $ 0.96 $				& $ 0.94 $    							& $ $                                              & $ $                     & $ 0.89 $   & $ 0.91 $\\
			$ \mathrm{TPR}_{0.01} $      & 	$ 0.87 $				& $ 0.85 $    							& $  $                                          & $  $                       & $ 0.7 $      & $ 0.75 $\\
			%			\hline
		\end{tabular}}
	\end{table*}



==> algorithm.tex <==
\section{Algorithm}
\label{sec:algorithm_ref}

In order to solve the source attribution problem, we need a reference fingerprint (the PRNU) that indexes each source camera, and a test fingerprint for the investigated query.

For the moment, let us focus on estimating  the PRNU of each source camera.
Actually, in multimedia forensic investigations, there is a strong probability of having available at court side manifold cameras, with the possibility of capturing photos or videos. 
In light of this, we propose 2 strategies for estimating the PRNU of each source camera, which can be alternatively pursued according to the specific situation: 
\begin{enumerate}[label=\textit{\Alph*)}]
	\item Estimating the reference PRNU from flat-field images shot by the camera.
	\item Estimating the reference PRNU from videos recorded by the camera, exploiting controlled and easily manageable sequences.  
\end{enumerate}
It follows an accurate description of the proposed methodologies. 

\input{alg_Ki}
\input{alg_Kv}





